Selective randomization inference for subgroup effects with continuous biomarkers

Randomization tests are a popular method for testing causal effects in clinical trials with finite-sample validity. In the presence of heterogeneous treatment effects, it is often of interest to select a subgroup that benefits from the treatment, frequently by choosing a cutoff for a continuous biomarker. However, selecting the cutoff and testing the effect on the same data may fail to control the type I error. To address this, we propose using "self-contained" methods for selecting biomarker-based subgroups (cutoffs) and applying conditioning to construct valid randomization tests for the subgroup effect. Compared to sample-splitting-based randomization tests, our proposal is fully deterministic, uses the entire selected subgroup for inference, and is thus more powerful. Moreover, we demonstrate scenarios where our procedure achieves power comparable to a randomization test with oracle knowledge of the benefiting subgroup. In addition, our procedure is as computationally efficient as standard randomization tests. Empirically, we illustrate the effectiveness of our method on simulated datasets and the German Breast Cancer Study.

==> power.tex <==
\section{Optimal subgroup}

We aim to identify a large subgroup that benefits from the treatment with high power.
First, notice that the largest subgroup benefiting from the selection is $\calS^* := \{i: \tau_i > 0\}$.
Below, we introduce our test statistic, and show that $\calS^*$ is also the subgroup with the maximal asymptotic power under a super-poluation model.
As a result, it is reasonable to choose $S^*$ as the optimal subgroup.


We start by describing the test statistic. 
We consider the following residual-based test statistic, motivated by \zg{Ref:Rosenbaum}. 
For the \(i\)-th unit, let \(\theta_i\) be the known propensity score, and we analyze the case where \(\theta_i = \theta\) \zg{(noting that the result can be generalized to heterogeneous \(\theta_i\))}. 
To begin, we estimate the marginal mean function, defined as \(\mu(w, x) := \mathbb{E}[Y_i \mid W_i = w, X_i = x]\), by fitting a regression model with \(Y\) as the response variable and \(W\) and \(X\) as the covariates. The choice of regression algorithm is flexible and can include methods such as linear regression, boosting, and neural networks.
Let \(\hat{\mu}(w, x)\) denote the estimator of the marginal mean function \(\mu(w, x)\). 
We then construct the test statistic as follows:
\begin{align}\label{eq:denoise}
    T(Z^*, W) = 
    % \frac{\sqrt{|\calS|}\sum_{i \in \calS} \psi_i}{\sum_{i \in \calS} (\psi_i - \sum_{i \in \calS} \psi_i/|\calS|)^2},
    \frac{\sum_{i \in \calS} \psi_i}{\sqrt{|\calS|}},
    \quad \psi_i := \frac{Z_i^* \left(Y_i - \hat{\mu}(W_i, X_i)\right)}{\theta} - \frac{(1-Z_i^*) (Y_i - \hat{\mu}(W_i, X_i))}{1-\theta}.    
\end{align}
We discuss reasons of the choice of the test statistic~\eqref{eq:denoise}.
Statistically, $\psi_i$ based on the residual \( Y_i - \hat{\mu}(W_i, X_i) \) is less variable than that based on the original response $Y_i$, which results in high power according to \Cref{prop:BerryEsseen}.
In fact, we show in a separate work that this test statistic with the true nuisance function $\mu(x)$ is more powerful than the augmented inverse propensity weighting (AIPW) test statistic for $\alpha$ small based on 
${Z_i^* \left(Y_i - \hat{\mu}_1(W_i, X_i)\right)}/{\theta} - {(1-Z_i^*) \left(Y_i - \hat{\mu}_0(W_i, X_i)\right)}/{(1-\theta)}$.
In addition, the nuisance estimation \(\hat{\mu}(w, x)\) needs to be executed only once, because \(\hat{\mu}(w, x)\) does not depend on \( Z_i \), and therefore remains unchanged when \( Z_i \) is replaced by the reassigned treatments \( Z_i^* \).
In contrast, the AIPW estimator requires fitting the nuisance functions \(\mu_0(x)\) and \(\mu_1(x)\) separately for each \(Z'\), making it computationally more demanding and less convenient.
 
\zg{Stopped here!!!}
We provide a power analysis of \eqref{eq:denoise}.
Define
\begin{align*}
    \sigma_i^2 = \var_{Z^*}(\psi_i) = \frac{1}{\theta(1-\theta)} (Y_i - \hat{\mu}(W_i, X_i))^2, \quad
    \rho_i = \EE_{Z^*}[|\psi_i|^3] = \frac{2 \theta^2 - 2 \theta + 1}{\theta^2(1-\theta)^2} |Y_i - \hat{\mu}(W_i, X_i)|^3.
\end{align*}
We first bound the distance between the reference distribution and the distribution of a standard normal.
\begin{proposition}\label{prop:BerryEsseen}
    For Bernoulli design with $\PP(Z_i = 1) = \theta$, 
    \begin{align*}
        \sup_{x \in \RR} \left|\PP_{Z^*}\left({T(Z^*, W)}\le x \right) - \Phi(x)\right| \le C \cdot \frac{\sum_{i \in \calS} \rho_i}{(\sum_{i \in \calS} \sigma_i^2)^{3/2}}.
    \end{align*}
    for some constant $0 < C < 0.56$, 
    % $v_g' = {\theta(1-\theta)}{\EE\left[\left(g(1,X_i,Y_i) - g(0,X_i,Y_i)\right)^2\right]}$.
    % Consequently, the asymptotic randomization distribution satisfies
    % \begin{align*}
    %     \frac{\bar{g}(Z')}{\sqrt{n v_g'}} \stackrel{d}{\to} \calN(0,1), \quad \frac{\bar{g}^N(Z')}{\sqrt{n}} \stackrel{d}{\to} \calN(0,1).
    % \end{align*}
\end{proposition}
In \Cref{prop:BerryEsseen}, only the reassigned treatment \( Z^* \) is considered random, while \( Y_i = Y_i(0) = Y_i(1)\), \( W_i \), and \( X_i \) are treated as fixed.  
% \Cref{prop:BerryEsseen} holds regardless of whether Fisher's sharp null hypothesis is true. However, under the sharp null hypothesis \( H_0: Y(1) = Y(0) + c \), the test statistic \( T(Z, W) \) is identically distributed as \( T(Z^*, W) \).  
Under the sharp null, $T(Z, W)$ should be of the same distribution of $T(Z^*, W)$, and is approximately normal.
The gap between the CDF of the test statistic and that of a standard normal converges at a parametric rate of \(n^{-1/2}\) (more precisely, the convergence rate is \(n^{-1/2} \cdot {\EE[\rho_i]}/{\EE[\sigma_i^2]}\)).
\Cref{prop:BerryEsseen} is proved by applying Berry-Esseen bound to $T(Z^*, W)$.


To calculate the asymptotic power, we need to analyze the asymptotics of the test statistic \( T(Z, W) \). 
We adopt the super-population model, where the potential outcomes are generated i.i.d. from the model 
$Y_i(j) = \mu_j(X_i) + \varepsilon_i$, $j \in \{0,1\}$,
with \(\varepsilon_i \independent (X_i, Z_i)\) and \(\mathrm{Var}(\varepsilon_i) = \sigma^2\). 
Provided with a nuisance function $\hat{\mu}(w, x)$, we define the nuisance function error $\delta_\mu(W_i, Z_i) = \hat{\mu}(W_i, Z_i) - \mu(W_i, Z_i)$.
Using \Cref{prop:BerryEsseen}, we quantify the power of the test as follows.
\begin{proposition}\label{prop:power.2}
    Under the super-population model with bounded \(\psi_i\), \(\rho_i / \sigma_i^3\), using the nuisance function $\hat{\mu}(w, x)$, then
    \begin{align}\label{eq:power.2}        
        \PP\left(P(Z, W) > \alpha\right) 
        \leq \Phi\left(-\frac{|\mathcal{S}|\mathbb{E}^2[\tau(W_i, X_i) \mid \mathcal{S}]}{\mathbb{E}[\tau^2(W_i, X_i) \mid \mathcal{S}] + \frac{\mathbb{E}[\delta_\mu^2(W_i, X_i) \mid \mathcal{S}] + \sigma^2}{\theta(1-\theta)}} + C_1 \log(|\calS|) \right) 
        + \frac{1}{|\mathcal{S}|} + C_2\sqrt{\frac{1}{|\mathcal{S}|}}.
        % \leq C_1 \left(\exp\left\{-C_2\frac{|\mathcal{S}|\mathbb{E}^2[\tau(W_i, X_i) \mid \mathcal{S}]}{\mathbb{E}[\tau^2(W_i, X_i) \mid \mathcal{S}] + \frac{\mathbb{E}[\delta_\mu^2(W_i, X_i) \mid \mathcal{S}] + \sigma^2}{\theta(1-\theta)}}\right\} + C_2\sqrt{\frac{1}{|\mathcal{S}|}} \right),
    \end{align}
    for constants \(C_1, C_2 > 0\).
\end{proposition}
We provide the proof sketch of \Cref{prop:power.2}.
Under the super-population model, \(T(Z, W)\) is a U-statistic. 
We apply concentration inequalities to \(T(Z, W)\) and calculate the p-value based on an exact standard normal reference distribution, which yields the first exponential term on the right-hand side of \eqref{eq:power.2}. 
Next, note that \Cref{prop:BerryEsseen} quantifies the distance of the reference distribution to a standard normal.
We bound \(\sum_i \rho_i\) and \(\sum_i\sigma_i^2\) used by \Cref{prop:BerryEsseen} again by concentraion inequalities and plug in \Cref{prop:BerryEsseen} to arrive at the second term on the right-hand side of \eqref{eq:power.2}. 


\Cref{prop:power.2} highlights how the power depends on the selected subgroup size $|\calS|$, magnitude of the treatment effect \(\EE[\tau(W_i, X_i) \mid \calS]\), second moment of the treatment effect \(\EE[\tau^2(W_i, X_i) \mid \calS]\), the accuracy of nuisance estimations \(\delta_\mu(W_i, X_i)\) in $\calS$, the noise level $\sigma^2$, and the propensity score $\theta$.
We use \Cref{prop:power.2} to guide the selection of subgroups \(\mathcal{S}\).
% In particular, we consider the simplified case where the individual treatment effect $Y_i(1) - Y_i(0)$ is observed.
% In this super-population model, this implies \(\sigma = 0\).
% Furthermore, we assume the true $\mu$ is available (accurate enought and this would be the most critical one.
\begin{proposition}\label{prop:subgroup}
    Under the super-population model, assuming the true \(\mu\) is provided, \(\sigma = 0\), the density of $\tau_i$ exists,
    % $f(t) = \lim_{\delta \to 0} (\PP(\tau_i \le t + \delta) - \PP(\tau_i \le t)) / \delta$, $t \in \RR$. 
    then among subgroups \(\calS(t) = \{i : \tau_i \geq t\}\), $\calS(0)$ achieves the maximal asymptotic power.
\end{proposition}


For $\sigma > 0$, we show in the proof of \cref{prop:subgroup} that the optimal threshold could be a positive number or zero (constant treatment effect). However, determining the exact value requires knowledge or estimation of the density \(f(t)\) and the noise magnitude \(\sigma^2\) for \(t > 0\). 
% Particularly for our method, we reserve the units with positive treatment effects for inference, and the selection is based on the screened-away individuals with negative treatment effects.  
As a result, we consider \(S^*\) as the oracle optimal subgroup, and our selection procedure aims to approximate it.


\begin{proof}[Proof of \Cref{prop:subgroup}]
    To maximize the asymptotic power, we maximize the core term $\frac{|\mathcal{S}|\mathbb{E}^2[\tau(W_i, X_i) \mid \mathcal{S}]}{\mathbb{E}[\tau^2(W_i, X_i) \mid \mathcal{S}]}$ in \Cref{prop:power.2}.
    Let $f(t)$ be the density of $\tau_i$, that is $f(t) = \lim_{\delta \to 0} (\PP(\tau_i \le t + \delta) - \PP(\tau_i \le t)) / \delta$.
    Then
    \begin{align*}
        |\calS| = n \int_{t}^\infty f(s) ds, \quad
        \EE[\tau(W_i, X_i)\mid \calS] = \frac{\int_{t}^\infty s f(s) ds}{\int_{t}^\infty f(s)}, \quad
        \EE[\tau^2(W_i, X_i)\mid \calS] = \frac{\int_{t}^\infty s^2 f(s) ds}{\int_{t}^\infty f(s)}.
    \end{align*}
    For $\calS(t)$,
    \begin{align*}
        \text{SNR}(t) 
        :=& \log\left(\frac{|\mathcal{S}(t)|\mathbb{E}^2[\tau(W_i, X_i) \mid \mathcal{S}(t)]}{\mathbb{E}[\tau^2(W_i, X_i) \mid \mathcal{S}(t)]}\right)\\
        =& \log\left(|\mathcal{S}(t)|\right) + \log\left(\mathbb{E}^2[\tau(W_i, X_i) \mid \mathcal{S}(t)]\right) - \log\left(\mathbb{E}[\tau^2(W_i, X_i) \mid \mathcal{S}(t)]\right) \\
        =& \log(n) 
        + 2\log\left(\int_t^\infty s f(s) ds\right) 
        - \log\left(\int_t^\infty s^2 f(s) ds\right). 
    \end{align*}
    We take derivative of $\text{SNR}(t)$ with regard to $t$, 
    \begin{align*}
        \text{SNR}'(t)
        =  -2\frac{t f(t)}{\int_t^\infty s f(s) ds}
        + \frac{t^2f(t)}{\int_t^\infty s^2 f(s) ds}.
        % \le  -2\frac{t f(t)}{\int_t^\infty s f(s) ds}
        % + \frac{tf(t)}{\int_t^\infty s f(s) ds} \le 0.
    \end{align*}
    For $t < 0$, $ \text{SNR}'(t) > 0$.
    For $t \ge 0$,
    \begin{align*}
         \text{SNR}'(t)
        \le  -2\frac{t f(t)}{\int_t^\infty s f(s) ds}
        + \frac{tf(t)}{\int_t^\infty s f(s) ds} \le 0,
    \end{align*}
    and the inequality can only be obtained iff $t = 0$.
    Therefore, the optimal threshold is $t = 0$, and $\calS(t)$ achieves the maximal asymptotic power.


    We discuss the case where $\sigma > 0$.
    \begin{align*}
        \text{SNR}(t) 
        &= \log(n) 
        + 2\log\left(\int_t^\infty s f(s) ds\right) 
        - \log\left(\int_t^\infty s^2 f(s) ds + \frac{\sigma^2}{\theta(1-\theta)} \int_t^\infty f(s) ds\right), \\
        \text{SNR}'(t) 
        &= -2\frac{t f(t)}{\int_t^\infty s f(s) ds}
        + \frac{t^2f(t) + \frac{\sigma^2}{\theta(1-\theta)} f(t)}{\int_t^\infty s^2 f(s) ds + \frac{\sigma^2}{\theta(1-\theta)} \int_t^\infty f(s) ds}.\\
    \end{align*}
    For \(t \leq 0\), \(\text{SNR}'(t) > 0\), which implies that the optimal threshold is a positive number.
\end{proof}




==> presentation.tex <==
1. intro: HTE, biomarker

Heterogeneous treatment effects, where treatment effects depend on individual characteristics, have gained significant interest in the past decade due to applications such as personalized medicine.
Given a treatment, there are two questions of interest: (1) identifying the subgroup that will benefit from the treatment; (2) testing the treatment's effectiveness among the selected subgroup.
Note that the subgroup selection typically will induce bias and require additional adjustment in the inference step.


Biomarkers, which are measurements of a biological condition, are a widely used and high-quality type of effect modifier. Typically, treatment effects are believed to vary monotonically with biomarkers, and without loss of generality, we assume that higher biomarker values are associated with more significant treatment effects.
We will explore cases beyond a single biomarker with monotone dependence towards the end.


2. dataset: GBCS trial
The German Breast Cancer Study Group (GBCS) trial 2 involves $473$ participants randomized into the treatment group with a hormone therapy and the control group without. 
% We analyzed 439 participants who had complete covariate data. 
The primary outcome measured was the time to the recurrence of breast cancer. The treatment effect is likely to be influenced by the biomarker: the number of progesterone receptors \parencite{stallard_adaptive_2023}, since the presence of more receptors increases the hormone absorption and thus enhances the treatment effectiveness.
It is natural to look for a subgroup whose number of progesterone receptors exceeds a data-driven threshold.


3. proposal overview + Figure 1 (GBCS data) + properties + GBCS data

We introduce a class of selection methods to find the subgroup benefiting from a treatment, utilizing a biomarker, and the inference therein.
For subgroup selection, we arrange units in ascending biomarker value order, sequentially reveal their outcomes, stop when the estimated treatment effect of the units with the current biomarker value exceeds zero (Stage 1 of \Cref{fig:diagram}), and select the units with biomarkers larger than the current value.
For inference, we simply apply the standard randomization test to the selected group (Stage 2 of \Cref{fig:diagram}).
Surprisingly, we prove that the testing method, with no apparent adjustment for the selection, controls the finite-sample type I error. 
Under the monotone dependence, we propose a specific selection approach  which will asymptotically yield the oracle subgroup consisting of all units benefiting from the treatment.
If the assumption of the monotone dependence between the treatment effect and the biomarker does not hold, the test is still valid and only the quality of the selected group is affected.


On the GBCS dataset in \Cref{sec:GBCS}, we testify our method using the number of progesterone receptors as the biomarker. 
Our approach selects the subgroup with more than $5$ progesterone receptors, resulting in a p-value of $0.0004$ for the null hypothesis of no treatment effect on the selected subgroup.
In comparison, if no selection is performed, the p-value for testing the null hypothesis of no treatment effect across the entire sample is $0.0037$;
In addition, when a FWER-control method is used to adjust for the selection, the p-value is $0.0411$.


4. Extensions, particularly the adaptive biomarker

\begin{itemize}
    \item Arc-shape dependence (\Cref{fig:extension} (a)).     
    % In addition to \Cref{assu:monotone}, there's a less common but still possible scenario where 
    In practice, it is possible that the effect of a new surgery might be stronger for older individuals but less effective, or even harmful, for very elderly people. 
    In this scenario, the treatment effect first increases and then decreases (arc-shape) as the biomarker value rises. 
    For this arc-shape dependence, we aim to find two thresholds $\hat{\lambda}_- < \hat{\lambda}_+$, and 
    select the subgroup $S_{\hat{\lambda}_-, \hat{\lambda}_+} = \{i: {\hat{\lambda}_-} < S_i < {\hat{\lambda}_+}\}$. 
    % The stopping time \(\hat{\lambda}_-\) is based on observations where \(S_i \leq S_{\hat{\lambda}_-}\), and \(\hat{\lambda}_+\) is based on observations where \(S_i \geq S_{\hat{\lambda}_+}\), which can be obtained by reversing \(X_i\). 
    % The p-value can be calculated in a similar manner while maintaining validity.
    We can apply the method for \Cref{assu:monotone} to $S_i$ and the sign-flipped $-S_i$ to obtain $\hat{\lambda}_-$ and $\hat{\lambda}_+$, respectively. 
    The inference method for $S_{\hat{\lambda}}$ remains valid for $S_{\hat{\lambda}_-, \hat{\lambda}_+}$.

    \item Multiple biomarkers (\Cref{fig:extension} (b)).
    In practice, it's possible that there are multiple biomarkers influencing a drug's effectiveness, such as the cholesterol level and BMI can collectively impact how effectively a medication lowers blood pressure. If this is the case, we can apply the method individually to each biomarker, resulting in multiple selected subgroups $\calS_{\hat{\lambda}_j}$, and take the intersection $\cap_{j} \calS_{\hat{\lambda}_j}$. The inference method for $S_{\hat{\lambda}}$ remains valid when applied to $\cap_{j} \calS_{\hat{\lambda}_j}$.
    
    \item Data-driven biomarker (\Cref{fig:extension} (c)).
    If no natural biomarker exists, we can utilize existing heterogeneous treatment effect estimators to build an artificial biomarker, such as genetic scores.
    
    Explicitly, we disclose a small subset of the data and train a treatment effect estimator to use as the data-driven biomarker. Subsequently, we reorder the units not yet utilized, reveal the outcomes of the next unit or batch, and stop if the estimated effect at the current data-driven biomarker satisfies a certain criterion. Otherwise, we update the data-driven biomarker and repeat from reordering.

\end{itemize}


(5. If interested, talk about the proof: partition defined by $G_\tau(z,w)$.)

==> previousApril2024.tex <==
\section{Introduction}\label{sec:introduction}

In a talk in 1956 titled ``Iterative Experimentation'', the great
statistician George Box suggested that we should keep in mind that
scientific research is usually an iterative process. He wrote in the
abstract:
\begin{quote}
  The cycle: conjecture-design-experiment-analysis leads to a new cycle
  of conjecture-design-experiment-analysis and so on. [...] Although this
  cycle is repeated many times during an inves-tigation, the experimental
  environment in which it is employed and the techniques appropriate for
  design and analysis tend to change as the investigation
  proceeds. \hfill \parencite{box1957}
\end{quote}
John Tukey, another great statistician and Box's contemporary,
acknowledged that Box's cycle ``will serve excellently'' if ``an
oversimple paradigm is to be selected'', but he noted that ``the point
where the circle is to be broken can be freely chosen'' and ``there
are short cuts and repeated steps as well as branchings and
rejoinings'' \parencite{tukey1963}.

Thus, although the demarcation in Box's cycle is very useful to
understand the role of statistical methodology in
different phases of experimentation, scientific research in the real
world does not always follow this linear process. Often, it is
desirable to continuously revise the scientific hypothesis and design
of the study as more data are gathered.
% When developing statistical methodology for practical problems, it is
% usually assumed that the scientific hypothesis and dataset are already
% given. However, real-world statistical problems are often much more
% complex, and it may be desirable to revise the hypothesis and design
% of the study as more data are gathered.
This has motivated two long-standing themes of research in statistics:
(i) \emph{selective inference}, where valid inference is required on potential
findings that are discovered after viewing the data, and (ii) \emph{adaptive
experimentation}, where data-adaptive designs are used to allow us to
collect more relevant data, save time and resources, and/or assign
more participants to a better treatment.

As the scale of datasets grows and increasingly precise conclusions are
sought, selective inference and adaptive experimentation have
attracted much attention in the recent literature. However, there is
strikingly little work on applying selective inference to adaptively
collected data. In this article, we will attempt to fill this gap and
develop a general method termed ``selective randomization inference''
that can be applied to a wide range of adaptive experiments. For the
rest of this section, we will first introduce our proposal and then
put it in the broader context set up by Box and Tukey.

\subsection{Overview of the selective randomization test}
\label{sec:overv-select-rand}


\begin{figure}[h]
  \centering
  \includegraphics[scale=0.185]{plot/two-stage-trial-graphic-03.pdf}
  \caption{Pictogram of a two-stage enrichment trial with two subgroups: low genetic risk score (green) and high genetic risk score (red).}
  \label{fig:trial-pictogram}
\end{figure}

Let us first use a hypothetical two-stage enrichment trial as a
running example to motivate the use of adaptive designs, illustrate
the potential pitfalls, and introduce our proposal (see also
Figure~\ref{fig:trial-pictogram}). This example is
motivated by a post hoc analysis by \textcite{marston_predicting_2020}
of the FOURIER trial (Further Cardiovascular Outcomes Researh With
PCSK9 Inhibition in Subjects With Elevated Risk). By partitioning
patients into different groups according to their genetic risk scores
for cardiovascular diseases, \textcite{marston_predicting_2020} found
that the new evolocumab therapy (PCSK9 inhibition) benefited patients
with high genetic risk much more than others. However, because of the
post hoc nature of this subgroup analysis, further randomized studies
may be required to confirm the conclusion.

Now consider a two-stage enrichment trial in which the patient
population is divided at the beginning of the study into a low
genetic risk group and a high genetic risk group. In the first stage
of the trial, patients are recruited from both groups and randomly
assigned the new therapy ($Z_{1i}=1$) or the placebo ($Z_{1i}=0$,
where $i$ is the patient index). Based on a preliminary analysis of
data from the first stage, we may wish to select one subgroup or both
subgroups for further investigation in the second stage. For
example, we may choose to only recruit people with high genetic risk
score if they show more promising responses in the first stage and potentially assign the new therapy with higher probabilities as well; let the treatment
assignment in the second stage be denoted by $Z_2$. We are interested
in testing whether there is any treatment effect for the subgroup(s)
selected at the end of the first stage, which is a categorical
variable denoted by $S_1 \in \mathcal{S}_1 = \{\text{only high}, \text{only low},
\text{both}\}$.

It has been recognized very early on that a naive analysis of such a
sequential trial tends to overstate statistical significance
\parencite{armitage_sequential_1960, anscombe_sequential_1963,
  pocock_group_1977}. To be more concrete, consider the following
randomization p-value that ignores selection. Let $Z = (Z_1,Z_2)$
denote all the treatment assignments and $W$ denote the recruitment
decisions, covariates and potential outcomes of the patients. A
randomization test conditions on $W$ and only uses the randomness in
the treatment assignment $Z$ to calculate the following p-value
\begin{equation*}\label{eq:rand-p-value}
  P_{\text{naive}} = \Prob(T(Z^*, W) \leq T(Z,W) \mid Z, W),
\end{equation*}
where $T(Z,W)$ is a test statistic that measures treatment efficacy
and $Z^* = (Z^{*}_1, Z^{*}_2)$ has the same distribution of $Z$ but is
conditionally independent of $Z$ given $W$. In this
definition, conditioning on $Z$ and $W$ means that the probability is
evaluated over the distribution of $Z^{*}$, an independent realization
of the treatment assignment. Due to subgroup selection,
$P_{\text{naive}}$ is generally not a valid p-value in the sense that
$\Prob(P_{\text{naive}} \leq \alpha)$ may be larger than the
significance level $0 < \alpha < 1$. This is because even though the
treatment assignment $Z$ is randomized, the selection ``changes'' its
distribution. Heuristically, suppose the high genetic risk group is
selected at the end of stage 1 (so $S_1 = \text{high}$), then the
first stage data must have already shown promises for the new therapy
in the high genetic risk group, and it is no longer appropriate to use
the randomization distribution of $Z_1$ to calculate the p-value. In
other words, it is ``unfair'' to compare $Z_1$ with $Z_1^*$ generated
from the original randomization distribution because $Z_1$ has gone
through selection but $Z_1^*$ does not.
A convenient solution to this problem is to discard the first stage,
aka data splitting \parencite{cox_note_1975}. That is, we use the data
of the first stage to choose the design and null hypothesis and the
second stage for statistical inference. Mathematically, this is equivalent to
conditioning on $Z_1^*=Z_1$, and in the context of randomization
inference, this amounts to using
\begin{equation*}\label{eq:2nd-stage-p-value}
  P_{\text{2nd\,only}} = \Prob(T(Z^*,W) \leq T(Z,W) \mid Z, W,
  Z_1^*=Z_1).
\end{equation*}
Obviously, this p-value is valid but uses the data in an inefficient
way.

In a nutsell, our proposal is to condition on the exact amount of
information used in the selection. This is inspired by the recent
literature on conditional post-selection inference, as will be
explained in \Cref{sec:related-work}. The key idea is that the selection
in the first stage $S_1 = S_1(Z_1, W)$ is a function of the treatment
assignment $Z_1$ and is thus a random variable. We argue that the
appropriate way to adjust for selection is to condition on it. This
leads to the following definition of the \emph{selective randomization
  test}: \taf{p-value?}
\begin{equation*}
  P_{\text{selective}}=\Prob(T(Z^*,W) \leq T(Z,W) \mid Z, W,
  S_1(Z_1^*, W)=S_1(Z_1, W)).
\end{equation*}
We will show that this p-value controls the selective type-I error in
the sense that
\begin{equation} \label{eq:selective-error}
  \Prob(P_{\text{selective}} \leq \alpha \mid W, S_1=s_1) \leq
  \alpha,\quad
  \text{for all}~s_1\in \calS_1~\text{and}~0 < \alpha < 1.
\end{equation}
Thus, no matter which subgroup is selected at the end of the first
stage, the false positive rate of this selective randomization test is
controlled. Compared to data splitting, this test is expected to be
more powerful because it uses the ``left out'' information in the
first stage that is not used by the selection.

\subsection{Related work}
\label{sec:related-work}

Our proposal is related to a wide range of research that offers
alternatives to the linear cycle of scientific research described by
Box. Next we will review the relevant literatures and compare them
with our proposal.

Adaptive designs can be traced back to the work of
\textcite{thompson_likelihood_1933} and are now frequently used in
many fields of empirical
research including medicine \parencite{burnett_adding_2020}, political
science \parencite{offer-westort_adaptive_2021}, and economics
\parencite{duflo_chapter_2007, kasy_adaptive_2021}. In many
situations, the experiments have several designated stages, and within
each stage the participants may be admitted on a rolling
basis. Therefore, preliminary data from the initial participants are
often available before the study concludes. This forms the basis for
adapting the treatment allocation or recruitment in later stages of
the experiment. For instance, it may be desirable to increase the
assignment probability of more promising treatments or policies
(this is called \emph{response-adaptive randomization}, see e.g.\
\textcite{rosenberger_covariate-adjusted_2001} and
\textcite{faseru_changing_2017}), discontinue certain arms of the study
early (this is called \emph{multi-arm multi-stage design}, see e.g.\
\textcite{magirr_generalized_2012} and \textcite{sydes_issues_2009}),
or focus on the subpopulation of participants that exhibit the best
reactions (this is called \emph{enrichment design}, see e.g.\
\textcite{magnusson_group_2013} and
\textcite{ho_efficacy_2012}). \taf{Comment: I cite one theoretical and one applied paper for the different designs each. Is this okay?} \textcite{pallmann_adaptive_2018}
provided an excellent review of adaptive designs in clinical trials
from a practical perspective.

Despite ethical advantages, logistical hurdles and statistical
challenges have prevented a wider adoption of adaptive designs
\parencite{robertson_point_2023} in clinical trials. This is because when Box's linear process of ``conjecture-design-experiment-analysis''
does not apply, most standard methods exhibit selection bias
\parencite{rosenberger_randomization_2015}. % For instance, in the
% enrichment trial we focus on a certain subpopulation in the second
% stage only if the first stage data already suggests that there is an
% effect. Hence, a naive analysis would be biased towards being
% significant. This issue was recognized early
% \parencite{armitage_sequential_1960, anscombe_sequential_1963,
% pocock_group_1977} and has been an active field of statistical
% research since.
% This problem has been considered in the clinical trials literature for
% decades.
For certain parametric models, the distribution of a test statistic in
an adaptive study can be derived \parencite{spencer_adaptive_2016,
  lin_inference_2021,frieri_design_2022}, or one can conduct hypothesis
tests for the different stages of the trial separately and combine the
resulting p-values \parencite{pocock_interim_1982,
  muller_adaptive_2001, stallard_adaptive_2023}.
However, these approaches are limited to just a few trial designs and
heavily rely on modelling assumptions that are often difficult to
justify. In the last decade, applications in online experiments
(of web services) sparked renewed interest in adaptively
collected data. A recent line of research uses adaptive weighting
techniques to recover asymptotic normality
\parencite{deshpande_accurate_2018, zhang_inference_2020,
  hadad_confidence_2021, zhang_statistical_2021}. In another novel
approach, \textcite{howard_time-uniform_2021} use martingale
concentration inequalities to construct any-time valid confidence
intervals for the average treatment effect. These new methods usually
require weaker assumptions but are often technically involved and only
apply to simple response-adaptive designs.

Selective inference seeks valid inference on potential findings that
are discovered after viewing the data
\parencite{benjaminiSelectiveInferenceSilent2020}. Several notions of
``validity'' (or selective risks) have been considered. The notion
with the longest history is familywise error, also known as
simultaneous inference, dating back to the
methods of \textcite{tukeyComparingIndividualMeans1949} and
\textcite{scheffeAnalysisVariance1959}. Although simultaneous
inference is often associated with multiple hypothesis testing, it can
also be applied to post-model selection problems
\parencite{berkValidPostselectionInference2013}. A more lenient notion
of risk
is the average error rate over the selected; examples include the
false discovery rate
\parencite{benjaminiControllingFalseDiscovery1995} and the false
coverage-statement rate
\parencite{benjaminiFalseDiscoveryRate2005a}. A third notion, which is
the one we use in the proposed selective randomization test, is the
conditional post-selection error
\parencite{fithian_optimal_2017}. This approach has seen a surge of
interest after successful applications to the model selection problem
\parencite{lee_exact_2016}; see
\textcite{kuchibhotla_post-selection_2022} for a recent review.
\taf{Do we want to distinguish between ``post-selection'' and ``selective''? I often see it used interchangeably but the former may be tied to model-selection a bit closer.}

\begin{figure}
  \centering
  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[r] & \text{design} \arrow[d] \\
      \text{analysis} \arrow[u] & \text{experiment} \arrow[l]
    \end{tikzcd}
    \caption{Box's cycle.}
    \label{fig:box}
  \end{subfigure}
  \quad
  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[r] & \text{design} \arrow[d, shift
      right = 1em] \\
      \text{analysis} & \text{experiment} \arrow[l] \arrow[u, shift
      right = 1em]
    \end{tikzcd}
    \caption{Response-adaptive randomization.}
    \label{fig:rar}
  \end{subfigure} \\[2em]

  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[r] & \text{design} \arrow[d] \\
      \text{analysis} & \text{experiment} \arrow[lu] \arrow[l]
    \end{tikzcd}
    \caption{Enrichment design.}
    \label{fig:enrichment}
  \end{subfigure}
  \quad
  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[d, shift right=1em] & \text{design} \arrow[d] \\
      \text{analysis} \arrow[u, shift right=1em] & \text{experiment} \arrow[l]
    \end{tikzcd}
    \caption{Selective inference.}
    \label{fig:posi}
  \end{subfigure} \\[2em]

   \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[r] & \text{design} \arrow[d] & \\
      \text{prelim analysis} \arrow[ur] & \text{experiment} \arrow[l] \arrow[r] & \text{final analysis}
    \end{tikzcd}
    \caption{Response-adaptive randomization (new).}
    \label{fig:rar-2}
  \end{subfigure} \\[2em]

  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[r] & \text{design} \arrow[d] \\
      \text{prelim analysis} \arrow[u] & \text{experiment} \arrow[l] \arrow[r] & \text{final analysis}
    \end{tikzcd}
    \caption{Enrichment design (new).}
    \label{fig:enrichment-2}
  \end{subfigure} \\[2em]
  
  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[drr] & \text{design} \arrow[d] & \\
      \text{prelim analysis} \arrow[u] & \text{experiment} \arrow[l] & \text{final analysis}
    \end{tikzcd}
    \caption{Selective inference (new).}
    \label{fig:posi-2}
  \end{subfigure} \\[2em]

  \begin{subfigure}[t]{0.4\textwidth} \centering
    \begin{tikzcd}
      \text{conjecture} \arrow[drr] \arrow[r] & \text{design} \arrow[d] \arrow[dr] & \\
      \text{prelim analysis} \arrow[u] \arrow[ur] & \text{experiment} \arrow[l] \arrow[r] & \text{final analysis}
    \end{tikzcd}
    \caption{Our problem.}
    \label{fig:ours}
  \end{subfigure}

  \caption{A schematic illustration of different
    modes of scientific research. Adaptive experimentation
    (\Cref{fig:rar,fig:enrichment}) and selective
    inference (\Cref{fig:posi}) break away from traditional
    statistical inference by inserting different ``mini cycles''
    within each cycle of conjecture-design-experiment-analysis
    described by \textcite{box1957}.}
  \label{fig:cycles}
\end{figure}

In view of Box's conjecture-design-experiment-analysis delineation of
scientific studies, adaptive experiments and selective inference
insert ``mini cycles'' within each study; this is illustrated in
\Cref{fig:cycles}. In adaptive experiments, preliminary data from the
experiment are used to modify the conjecture (\Cref{fig:rar}) and
experimental design (\Cref{fig:enrichment}). In selective \taf{post-selection?} inference,
preliminary analyses (e.g.\ a model selection procedure) are used to
modify the conjecture (\Cref{fig:posi}). As mentioned previously, the
proposed selective randomization test is an application of selective
inference, particularly conditional post-selection inference, to
adaptive experiments. % This properly addresses the selection bias
% arising from the adaptive design.

Two points merit a discussion at this point. First, among the
different approaches to selective inference, we believe conditional
inference is the most appropriate for adaptive clinical trials. This
is because controlling the selective type I error as in
\eqref{eq:selective-error} allows us to \emph{treat the selected
  hypothesis as given} when interpreting the results. This is crucial
in objectively evaluating the evidence in a randomized experiment from
a regulatory perspective. The familywise error rate is unnecessarily
strict as we are often just interested in testing one hypothesis, and
the more lenient notions such as the false discovery rate are more
suitable for discovering promising hypotheses and less suitable for
confirmatory studies.

Second, compared to existing methods for inference after model
selection, a distinguishing feature of the selective randomization
test is that it is model-free. In particular, it does not require any
parametric model on the outcome, not even that the data points are
independent or identically distributed. Originally suggested by
\textcite{fisher_design_1935} and elaborated by
\textcite{pitman_significance_1937}, randomization inference is
exactly based on the randomness introduced by the experimenter, or in
Fisher's words, the ``physical act of randomization'' justifies the
statistical inference. Although model-based inference are predominant
in the analyses of randomized experiments, interest in randomization
inference has rekindled in recent years especially for complex designs
\parencite{ji_randomization_2017,
  rosenberger_randomization_2019,wang_randomization_2020,
  offer-westort_adaptive_2021, bugni_inference_2018}. Some previous works
examined the use of randomization inference in adaptive
experiments \parencite{edwards_model_1999,simon2011using}, but the
selective randomization test proposed here can be applied to a much
wider class of adaptive designs.

\taf{ORGANIZATION OF THE PAPER}


\section{Adaptive Multi-stage Studies}\label{sec:notation}
In this work, we consider fully adaptive studies with $K$ stages and $L+1$ different treatments, e.g.\ drugs, types of therapy, dosages of a certain drug etc., enumerated from $0$ to $L$. At every stage both the recruitment of participants and the treatment assignment mechanism may depend on the data observed in previous stages. This section introduces the set-up of the trial and the notation used in this article. In the following, $k\in\{1,\ldots,K\}$ denotes an arbitrary stage and $l \in \{0,\ldots,L\}$ an arbitrary treatment.

We use the following standard notations. Participants are recruited from a pool of $n$ candidates. For each such candidate $i \in \{1,\ldots,n\}$, covariate information $X_i$ is available; we set $X := (X_i)_{i\in \{1,\ldots,n\}}$. The effect that treatment~$l$ has on a unit~$i$ is captured by the potential outcome $Y_i(l)$. All potential outcomes of one participant $i$ are denoted by $Y_i(\cdot) := (Y_i(l))_{l}$ and the potential outcomes of the pool of candidates by $Y(\cdot) := (Y_i(\cdot))_{i \in \{1,\ldots,n\}}$. Here, we implicitly make the familiar assumption of ``no interference''. This means that the potential outcomes of one participant does not depend on the treatments that other people receive. Moreover, we introduce the notations $X_I := (X_i)_{i \in I}$ and $Y_I(\cdot) := (Y_i(\cdot))_{i \in I}$ for $I\subseteq \{1,\ldots,n\}$.

Unlike many standard designs, the decision which participants to recruit may depend on previously observed data. To explicitly describe this feature of adaptive studies we model the recruitment decisions via the random sets $R_1, \ldots, R_K \subseteq \{1,\ldots,n\}$. These contain the indices of participants that are recruited in the different stages. We require that each unit can be included into the trial at most once; this implies that all $R_1,\ldots, R_K$ must be disjoint. Note that this work does not consider longitudinal studies with patient follow up over multiple time points. %The recruitment decisions at the different stages are based on the covariate information and data observed in previous stages.
The covariates and potential outcomes of participants at stage $k$ are denoted by $X_{R_k}$ and $Y_{R_k}(\cdot)$, respectively. Moreover, we use the notation ${R:= \cup_k R_k}$.

At stage $k$, the recruited units are administered the treatments $Z_k \in \calZ_k \subseteq \{0,\ldots,L\}^{\lvert R_k\rvert}$ whose distribution may depend on the covariates of the recruited participants $X_{R_k}$. %Note that $Z_k$ is the whole random vector of assigned treatments and that its support $\calZ_k$ can be constrained, for instance by requiring that all treatments are equally often administered.
The treatment assignment determines which of the potential outcomes is actually realized: the observed values of the outcome variable are denoted by $Y_{R_k}$. We assume consistency which ensures that the observed values equal the potential outcomes under the realized treatment assignment, i.e.\ $Y_{R_k} = Y_{R_k}(Z_k)$.
% \begin{equation*}
%   Y_{R_k} = Y_{R_k}(W_k) := (Y_{R_{k,i}}(W_{k,i}))_{i \in \{1,\ldots,\lvert R_k\rvert\}}.
% \end{equation*}
In the following, we use the short-hands $Z = (Z_k)_k$, $\calZ = \bigtimes_k\, \calZ_k$ and $Y_R$.

The second characteristic feature of our setting are the selection statistics $S_k$. After administering the treatment and recording the response in stage $k$, the experimenters analyse the data from stages $1$ through $k$ and compute the value of $S_k$ which encapsulates the information that is passed on to stage $k+1$. This is typically the chosen design of stage $k+1$. Importantly, both the recruitment decisions and the treatment assignment at any given stage $k+1$ can only depend on previous stages through the selection statistic $S_{k}$. After completing the trial, the researchers choose a null hypothesis that may depend on the observed data of all stages of the trial. Hence, we model it as the final selection statistic $S_K$. We set $S:=(S_1,\ldots,S_K) \in \calS = \calS_{-K}\times \calS_K$. To emphasize the dependence of $S$ on $W$, we write $S(W)$.

\begin{figure}[t] \centering
  \begin{tikzpicture}
    % Stage I
    \node at (0,0) (yr1) {$Y_{R_1}$};
    \node at (-2,1.5) (xr1) {$R_1,X_{R_1}$};
    \node at (-2,-1.5) (w1) {$Z_1$};
    \node at (2,0) (s1) {$S_1$};
    \node at (0,2) (yr1s) {$Y_{R_1}(\cdot)$};

    % Stage II
    \node at (6,0) (yr2) {$Y_{R_2}$};
    \node at (4,1.5) (xr2) {$R_2,X_{R_2}$};
    \node at (4,-1.5) (w2) {$Z_2$};
    \node at (8,0) (s2) {$S_2$};
    \node at (6,2) (yr2s) {$Y_{R_2}(\cdot)$};

    % Population
    \node at (3,3.75) (ys) {$Y(\cdot)$};
    \node at (0.5,3.75) (x) {$X$};
    % \node at (1.75,4.75) (u) {$U$};

    % Population
    \draw[-latex, thick] (x) -- (ys);
    % \draw[-latex, thick] (u) -- (x);
    % \draw[-latex, thick] (u) -- (ys);


    % Stage I
    \draw[-latex, thick] (xr1) -- (w1);
    \draw[-latex, thick] (w1) -- (yr1);
    \draw[-latex, thick] (yr1) -- (s1);
    \draw[-latex, thick] (xr1) -- (s1);
    \draw[-latex, thick] (w1) -- (s1);
    \draw[-latex, thick] (x) -- (xr1);
    \draw[-latex, thick] (xr1) -- (yr1s);
    \draw[-latex, thick] (yr1s) -- (yr1);
    \draw[-latex, thick] (ys) -- (yr1s);

    % Stage II
    \draw[-latex, thick] (xr2) -- (w2);
    \draw[-latex, thick] (w2) -- (yr2);
    \draw[-latex, thick] (yr2) -- (s2);
    \draw[-latex, thick] (xr2) -- (s2);
    \draw[-latex, thick] (w2) -- (s2);
    \draw[-latex, thick] (x) -- (xr2);
    \draw[-latex, thick] (xr2) -- (yr2s);
    \draw[-latex, thick] (yr2s) -- (yr2);
    \draw[-latex, thick] (ys) -- (yr2s);

    % Inter stages
    \draw[-latex, thick] (s1) -- (xr2);
    \draw[-latex, thick] (s1) -- (w2);

    \draw[-latex, thick, color=black] (s1) .. controls (2.2,-3.2) and (7.5,-3.2) .. (s2);
    % \draw[-latex, thick, color=black] (yr1) .. controls (2.2,-3.5) and (7.7,-3.5) .. (s2);
    % \draw[-latex, thick, color=black] (xr1) .. controls (0.5,-4) and (7.9,-4) .. (s2);
    % \draw[-latex, thick, out=-15, in=-90,color=black] (w1) .. controls (0.5, -3.1) and (8.1, -4.5) .. (s2);

    % Background
    \begin{pgfonlayer}{background}
      \node [fill=blue!20,fit=(w1) (yr1s) (xr1) (yr1), text=blue, align=right,text height=115pt] {\phantom{blabla}Stage 1};
      \node [fill=blue!20,fit=(w2) (yr2s) (xr2) (yr2), text=blue, align=right, text height=115pt] {\phantom{blabla}Stage 2};
      \node [fill=red!20,fit=(s1)] {};
      \node [fill=red!20,fit=(s2)] {};
      \node [fill=black!20,fit=(x) (ys)] {};
    \end{pgfonlayer}

  \end{tikzpicture}
  \caption{Directed acyclic graph (DAG) of a two-stage adaptive trial. In addition, $S_2$ may directly depend on the observed data from the first stage: $X_{R_1}, Z_1$ and $Y_{R_1}$. For simplicity, these relationships are not depicted.}
  \label{fig:dag}
\end{figure}

In order to describe the relationships between the different variables we use a directed acyclic graph (DAG). Figure~\ref{fig:dag} depicts a generic adaptive two-stage trial; analogously, the DAG can be extended to $K$ stages. We represent $R_k$ and $X_{R_k}$ as one node to ease readability. Under the Markov assumption, we can directly read off conditional independence relationships from the DAG \parencite{spirtes_2000}.

\begin{remark}
  In general, the DAG is not faithful to the underlying probability distribution as it includes deterministic relationships. For instance, $Y_{R_k}$ is a deterministic function of $Z_k$ and $Y_{R_k}(\cdot)$. For our purposes, though, this does not pose a problem as we only rely on the conditional independences obtained from the Markov assumption. For a thorough discussion of determinism and faithfulness we refer to \textcite[chap. 2--3]{spirtes_2000}.
\end{remark}



\section{Selective Randomization Inference}\label{sec:selective-inference}
This section applies ideas from the selective inference literature to randomization inference in adaptive studies. We formally introduce the selective randomization p-value and address estimation of a homogeneous treatment effect and the construction of confidence intervals.


\subsection{Selective Randomization Distribution}
Randomization inference leverages the fact that the distribution of the treatment assignments $Z$ is chosen by the experimenter and is thus known. In order to avoid imposing modelling assumptions on the potential outcomes and covariates that may be unrealistic, we condition $Z$ on these quantities. In most settings, the choice of units to include into the study is fixed and therefore not explicitly pointed out. In adaptive studies, however, the recruitment of participants $R$ may depend on the treatment assignments $Z$. To ensure that we conduct inference only for the units observed in the realized study, we additionally condition on $R$. This yields the randomization distribution $Z \,\vert\, R, X_R, Y_R(\cdot)$; in the following, we use the abbreviation
\begin{equation*}
  W := (R, X_R, Y_R(\cdot)).
\end{equation*}
Note that $Z$ is conditionally independent of the covariates and potential outcomes of not recruited units according to the DAG, cf.\ Figure~\ref{fig:dag}.


% traditional randomization inference conditions on these quantities. Thus, we obtain the randomization distribution of the treatment assignments: $Z\,\vert\, X, Y(\cdot)$.

% This, implicitly assumes that the units participating in the trial are always the same -- regardless of the treatments assigned. In our setting, however, the recruitment of participants $R$ is adaptive and modelled explicitly. In fact, we do not observe any potential outcome and may not even know the covariates of the candidates $\{1,\ldots,n\}\setminus R$ that were not included into the trial. To ensure that we conduct inference for observed units only, we additionally condition the randomization distribution on $R$.

% According to the DAG, this implies that $Z$ is conditionally independent of the covariates and potential outcomes of not recruited participants. This yields the randomization distribution $Z \,\vert\, R, X_R, Y_R(\cdot)$. In the following, we will use the abbreviation $W := (R, X_R, Y_R(\cdot)) \in \calW$.


Under a suitable null hypothesis -- see the following section --, $W$ is known and we may try to use the randomization distribution $Z\mid W$ to conduct inference. Yet, this approach does generally not provide the statistical guarantees we seek. Since the choice/selection of the model, i.e.\ the distribution of $Z\mid W$, and null hypothesis is data-dependent in adaptive studies, it usually carries information about the validity of the null hypothesis. In other words, we may often encounter the situation where we would test the null hypothesis of ``no effect'' only when the data has already suggested that there is an effect. To remove any information about the null hypothesis contained in the selection, \textcite{fithian_optimal_2017} \taf{cite other papers?} propose to condition on the selective choice.
% They state their guiding principle as follows:
% \begin{displayquote}
%   \centering
%   \textit{
%   The answer must be valid, given that the question was asked.
% }
% \end{displayquote}
This principle likewise applies to estimation and the construction of confidence intervals. The choice of null hypothesis is captured by the statistic $S_K$. The choice of model, on the other hand, is more subtle. According to the conditional independence relationships that can be read off the DAG, we can decompose $Z\,\vert\, W$ as follows
\begin{align*}
  % \Prob(W = w\mid R=r,X_R=x_r,Y_R(\cdot)=y_r) &=
    \Prob(Z_1=z_1,\ldots,Z_K=z_K\mid W=w)
    &= \prod_{k=1}^K \Prob(Z_k = z_k \mid W=w, Z_1=z_1,\ldots, Z_{k-1} = z_{k-1})\\
    &=\prod_{k=1}^K \Prob(Z_k = Z_k \mid W=w, S_{k-1}= s_{k-1}),
\end{align*}
where we use the convention $S_0 := \emptyset$. This shows that space of all models for $Z$ can be identified with $\calS_{-K}$. Hence, we also condition on the statistics $S_1,\ldots,S_{K-1}$. This yields the selective randomization distribution $Z\,\vert\, W,S(Z)$ which will be used in the following two sections to conduct inference.

%\begin{remark}
%Since $S$ is a function of $W$ and $Z$ and $W$ has a discrete distribution, $\Prob(S = s\mid Z=z) > 0$ holds for all $s \in \calS$ and $z \in \calZ$. Hence, the conditional distribution above is well-defined. If $S$ captures most of the information of $W$, we condition on an event with small probability which leads to a decrease in power; see further subsection \ref{sec:confint}. \taf{change last sentence}
%\end{remark}

\subsection{Hypothesis Testing}\label{sec:hypothesis-testing}

After concluding the trial, we analyse the effectiveness of the studied treatments by comparing different potential outcomes. Since we observe only one potential outcome for every recruited participant, the null hypothesis typically relates the realized outcomes $Y_R$ to (a subset of) the full potential outcomes $Y_R(\cdot)$ and thus allows us to impute (a subset of) $Y_R(\cdot)$ from $Y_R$. A common hypothesis in randomization inference is the fully sharp null:
\begin{equation*}%\label{eq:sharp-null}
    \mathrm{H}_0:\quad Y_i(l)=Y_i(l'),\quad \text{for all } l,l'\in \{0,\ldots,L\},\, i \in R.
\end{equation*}
Under this hypothesis, all potential outcomes can be imputed from the observed outcomes and we can directly use the selective randomization distribution to conduct inference.

Yet, in many adaptive studies the null hypothesis of interest is only partially sharp, meaning that only a subset of the potential outcome schedule $Y_R(\cdot)$ can be imputed from $Y_R$. For instance, we may like to test the effect of the treatments only in a specific subgroup, e.g.
\begin{equation*}%\label{eq:partial-null-1}
    \mathrm{H}_0:\quad Y_i(l)=Y_i(l'),\quad \text{for all } l,l'\in \{0,\ldots,L\},\, i \in R: X_i\geq 0.
\end{equation*}
or only consider a subset of treatments, e.g.
\begin{equation*}%\label{eq:partial-null-2}
    \mathrm{H}_0:\quad Y_i(0)=Y_i(1),\quad \text{for all } i \in R.
\end{equation*}
In the first example, we can conduct inference by discarding units that are not part of the subgroup of interest; in the second example, we need to restrict $Z$ to only take values in $\{0,1\}$. For a general partially sharp null hypothesis, we usually need to condition the selective randomization distribution on an additional statistic $G(Z):=G(Z,W)\in \calG$. For a partially sharp null hypothesis in a subgroup or subset of treatments, we use
$G(Z) = (Z_{k,i}\colon X_{k,i} < 0)_{k,i}$ or $G(Z) = (Z_{k,i}\cdot\one\{Z_{k,i} \notin \{0,1\}\})_{k,i}$, respectively.

In summary, we use the distribution of $Z\mid W,S(Z),G(Z)$ to conduct inference; we condition on $S$ to account for the selection of design and null hypothesis and on $G$ to accommodate partially sharp null hypotheses. In general, the choice of statistic that is used to test the selected null hypothesis can depend on the values of $S$ and $G$. Therefore, we consider a collection of statistics $(T_{s,g})_{s\in\calS, g\in\calG}$, where each $T_{s,g}$ is a function of $W$ and $Z$. Based on the selective randomization distribution of the test statistic given by
\begin{equation*}
    T_{S,G}(Z,W)\mid W, S(Z), G(Z),
\end{equation*}
we define the selective randomization p-value.


\begin{definition}\label{def:rand-p-value}
    In the setting above, let $Z^*$ have the same distribution as $Z$ and fulfill $Z^*\indep Z\,\vert\,W$. Then, the \emph{selective randomization p-value} is given by
    \begin{equation}
        p(Z,W):=\Prob^*\Big(T_{S,G}(Z^*,W) \leq T_{S,G}(Z,W) \,\Big\vert\, W, Z, S(Z^*) = S(Z), G(Z^*) = G(Z)\Big).\label{eq:rand-p-value}
    \end{equation}
\end{definition}

Note that the selective randomization p-value is a specific instance of the conditional randomization p-value of \textcite{zhang_2023_randomization_test}. Therefore, its validity follows immediately.

\begin{proposition}\label{thm:type-i-error}
    Let $\alpha \in [0,1]$. The selective randomization p-value as given in Definition \ref{def:rand-p-value} stochastically dominates the uniform distribution on $[0,1]$:
    \begin{equation*}
        \Prob(\,p(Z,W) \leq \alpha \,\vert\, W, S(Z)=s, G(Z)=g) \leq \alpha\quad \forall\, s\in \calS, g\in \calG.
    \end{equation*}
    Consequently, a test which rejects the selected null hypothesis when $p(Z,W) \leq \alpha$ controls the selective type-I error, that is
    \begin{equation*}
        \Prob(\,p(Z,W) \leq \alpha \mid W, S(Z)=s) \leq \alpha\quad \forall\, s\in \calS.
    \end{equation*}
\end{proposition}
\begin{proof}
    See \textcite[Thm.\ 1]{zhang_2023_randomization_test}, where the partition of the treatment assignment space $\calZ$ is given by the preimages of $(S,G)$, cf.\ \textcite[Prop.\ 1]{zhang_2023_randomization_test}.
\end{proof}

\begin{remark}
    \textcite{simon2011using} consider trials where the recruitment is non-adaptive and the treatment assignment distribution may depend on previous stages. They prove that the usual randomization p-value is valid under the assumption
    \begin{equation}\label{eq:simon-assumption}
        (Z_1,\ldots, Z_{k-1})\indep (X_k, Y_k) \mid (X_1,Y_1),\ldots,(X_{k-1},Y_{k-1}),\qquad \text{for all }k \in \{1,\ldots,K\}.
    \end{equation}
    Their result is a special case of Proposition~\ref{thm:type-i-error} as \eqref{eq:simon-assumption} implies that any $S_k$ can be a function of only $(X_1,Y_1),\ldots,(X_{k},Y_{k})$ but not $(Z_1,\ldots,Z_k)$. Hence, we can drop $S$ in the definition of the selective randomization p-value \eqref{eq:rand-p-value} as $X$ and $Y$ are also conditioned on and thus recover the usual randomization p-value.
\end{remark}

When randomization inference is applied in practice, $S$ is stipulated by the experimenters before executing the trial, whereas $G$ and the test statistics $(T_{s,g})_{s,g}$ are chosen by the statisticians analysing the trial after its completion. If the selected null hypothesis is partially sharp, only a subset of the potential outcomes $Y_R(\cdot)$ of the recruited participants can be imputed from the observed outcomes $Y_R$. Since the selective randomization p-value generally depends on all potential outcomes, this raises the question whether it can actually be computed. To ensure this, statisticians need to choose the test statistics $(T_{s,g})_{s,g}$ and $G$ such that the former only depend on potential outcomes that can be inferred from the selected null hypothesis. Accordingly, such statistics are called \emph{imputable}; for a more detailed discussion, we refer to \textcite{zhang_2023_randomization_test}.
\taf{not completely happy with the paragraph above}


\subsection{Confidence Intervals and Estimation}\label{sec:confint}
Thus far, we have focused on conducting hypothesis tests. Yet, our proposed selective randomization p-value can also be used to construct confidence intervals and estimators for a homogeneous treatment effect $\tau$. This effect is usually defined as the differences between the potential outcomes under two treatments $l$ and $l'$ in a subset of the recruited units $I$.
The associated null hypothesis is given by
\begin{equation*}
    \mathrm{H}_0^\tau\colon\quad Y_i(l)-Y_i(l') = \tau\quad \forall\, i \in I\subseteq R.
\end{equation*}
and the corresponding selective randomization p-value is denoted by $p_\tau(Z)$. (Note that we can equally define the homogeneous treatment effect $\tau$ across more than two treatments.)

Due to the duality of hypothesis testing and confidence sets, we can simply invert the selective hypothesis tests for different values of $\tau$ to construct the confidence set
\begin{equation*}\label{eq:confidence-set}
        C_{1-\alpha}(Z) := \{\tau \in \RR\colon p_\tau(Z) > \alpha\}.
\end{equation*}
\begin{lemma}
    Let $\alpha \in [0,1]$. If there exists a $\tau_0$ such that the hypothesis $\mathrm{H}_0^{\tau_0}$ is true, then
    $C_{1-\alpha}(Z)$
    is a selective $1-\alpha$ confidence set, that is
    \begin{equation*}
        \Prob(\tau_0 \in C_{1-\alpha}(Z)\mid W,S(Z)=s)\geq 1-\alpha\quad \forall\,s \in \calS.
    \end{equation*}
\end{lemma}

\begin{proof}
By definition of the confidence set and Proposition \ref{thm:type-i-error}, we obtain
    \begin{equation*}
        \Prob(\tau_0 \notin C_{1-\alpha}(Z)\mid W,S(Z)=s) =
        \Prob(p_{\tau_0}(Z) \leq \alpha\mid W,S(Z)=s) \leq \alpha\quad \forall\,s\in \calS.
    \end{equation*}
\end{proof}
Applying a similar reasoning, we can estimate the homogeneous effect as the $\tau$-value that achieves a selective randomization p-value of $1/2$, i.e.\ $\hat{\tau} = \tau$ such that $p_\tau(Z) = 1/2$. Since it may be impossible to find a value of $\tau$ that fulfills this condition exactly, the Hodges-Lehmann (HL) estimator \parencite{jr_estimates_1963, rosenbaum_hodges-lehmann_1993} is defined as follows
\begin{equation*}\label{eq:hl-estimator}
    \hat{\tau} = \frac{\sup\{\tau\colon p_\tau(Z)< 1/2\}+\inf\{\tau\colon p_\tau(Z)> 1/2\}}{2}.
\end{equation*}

When the p-value $p_\tau(Z)$ is monotonically increasing in $\tau$, the curve $\tau \mapsto p_\tau(Z)$ crosses every level exactly once. Consequently, the proposed confidence set and estimator are ``well-behaved'': $C_{1-\alpha}(Z)$ is an \emph{interval} and the HL estimator is the intuitively correct definition of a point estimator. \taf{not happy with the HL part} For unconditional randomization inference, \textcite{caughey_randomisation_2023} provide conditions under which the corresponding p-value is indeed monotone. Yet, when we condition on the selection event, the p-value curve is generally not monotone. Heuristically, if we test increasingly extreme values of $\tau$, there are often fewer and fewer alternative treatment assignments $z^*$ that lead to the same selective choices as in the original trial, i.e.\ $S(z^*) = S(Z)$. Therefore, the p-value curve becomes increasingly jagged. Hence, the confidence set defined via inversion of tests may be disconnected and the p-value curve may cross the level $1/2$ multiple times complicating the definition of a point estimator. We demonstrate this phenomenon with the two-stage trial example from the introduction. More details on this simulation study can be found in Section~\taf{insert number} and Appendix~\taf{add appendix}. When the selection of the null hypothesis depends on data from the first \emph{and} second stage, the first panel of Figure~\ref{fig:hold-out} shows that the p-value curve may be far from monotone. For instance, it crosses the level $1/2$ six times yielding six potential point estimates.

\begin{figure}
        \centering
        \includegraphics[scale=0.6]{plot/hold-out-plots.pdf}
        \caption{Smoothing effect of hold-out units. In the first panel, the p-value curve (green) is plotted for a selection rule that uses stage I and II units; in the second panel, only stage I units are used for selection; in the third panel, only stage I units are used for selection but inference is based on the second stage randomization p-value, cf.\ data splitting. The true treatment effect equals 1 in this simulation.}
    \label{fig:hold-out}
\end{figure}

To mitigate the risk of a jagged p-value curve and the resulting difficulties of interpreting the inference results, we propose the use of \emph{hold-out units}. These units are not taken into account when making selective choices; for example, the experimenters may decide on the null hypothesis before gathering data from the participants in the last stage of the study. Since $S$ does not depend on the treatments assigned to hold-out units, the number of alternative treatments $z^*$ cannot sink below a certain threshold -- even for extreme values of $\tau$. In the second panel of Figure~\ref{fig:hold-out}, we plot the p-value curve when only the first stage data is used for selection of the null hypothesis and the second stage participants serve as hold-out units. The curve is not monotone but clearly smoother and yields a unique point estimate and $90\%$ confidence interval.


\include{computation}
%\section{Computation}\label{sec:computation}

%Note on separability concerning the dotted edges

%\taf{Rejection sampling and MCMC generate samples from a target distribution. We are in the special case that we know the distribution of $W$ and can directly sample from it but $W\mid G(W)=g,S(W)=s$ is more complicated. Hence, for $w$ such that $G(w)=g$ and $S(w)=s$, we have $\Prob(W=w\mid G(W)=g, S(W)=s) = C\cdot \Prob(W=w)$, where $C\geq 1$ and the same for all $w$.

%Is this useful?
%}

%\subsection{Rejection Sampling}

%\subsection{Markov Chain Monte Carlo}

%\subsection{Confidence Sets}\label{sec:comp-confidence-sets}


% \section{Examples}

\section{Discussion and Outlook}

%In many modern studies, researchers conduct one or multiple preliminary data analyses that inform the further design of the experiment and/or the conjecture. This helps them use resources more efficiently, make more ethical decisions and tailor the experiment to their needs. While this flexibility is desirable for practitioners, standard statistical methods cannot accommodate an interim data analysis, cf.\ Box's cycle. \taf{linear process} \taf{Cut the paragraph above?}

To analyse data from adaptive studies, we use the paradigm of randomization inference as it has two major benefits. First, randomization inference does not require any modelling assumptions on the distribution of the covariates and outcomes or the ubiquitous condition of i.i.d.\ data points. Therefore, it is an ideal default tool for conducting inference that can stand on its own or complement a model-based analysis. Second, randomization inference naturally lends itself to handle selective choices. Recent model-based proposals typically involve considerable technical difficulties and can only be used for specific types of adaptive studies. On the other hand, our proposed selective randomization p-value can accommodate all kinds of selective choices. The reason for this flexibility stems from the following insight: In standard randomization inference, we compare the realized treatment assignment $Z$ to all alternative assignments $Z^*$; in adaptive studies, however, it is only fair to compare to $Z^*$ that lead to the same choices as in the original trial. Hence, conditioning on the information expressed in the selection, i.e.\ conditioning on $S(Z^*)=S(Z)$, suffices to provide valid inference. This holds true regardless of the type of selective choice.

While this article is mainly concerned with introducing selective randomization inference and exploring some immediate questions like constructing confidence intervals or computing the p-value, there are many conceivable extensions.

First, we only consider the classical case of a (partially) sharp null hypothesis in this work. This implies testing that the treatment effect is the same for every (or a subgroup of) individual in the study. Since such null hypotheses are sometimes criticized as overly restrictive and therefore of little interest to practitioners, many recent articles focus on relaxing the sharp null. \textcite{caughey_randomisation_2023} propose to test one-sided null hypotheses; another line of research considers weak null hypotheses that concern the average treatment effect among the participants \parencite{ding_paradox_2017, wu_randomization_2021, cohen_gaussian_2022}. Moreover, standard treatment assignment mechanisms, e.g.\ completely randomized or Bernoulli trials, may lead to covariate imbalance between different arms of the study. To remedy this issue, rerandomization tests \parencite{morgan_rerandomization_2012, wang_rerandomization_2022} condition the distribution of $Z$ on a balance criterion. Integrating these recent developments %on alternative null hypotheses and rerandomization
into our selective randomization inference framework, would greatly add to its flexibility and appeal.% of the presented approach.

Second, this work is mainly targeted to adaptive studies that use a selection statistic $S$ that takes discrete values. Conceptually, there is no obstacle to apply our method to continuous selection rules. However, the selective randomization p-value may reduce to the data splitting p-value. Consider our running example of a two-stage enrichment trial: In the extreme case that each first-stage treatment assignment leads to a different value of the selection statistic $S(Z_1)$, conditioning on $S(Z_1^*)=S(Z_1)$ is equivalent to conditioning on $Z_1^* = Z_1$. Even when there are a few first-stage treatment assignments yielding the same value of a continuous selection statistic, it is computationally hard to identify them, especially when rejection sampling is used. These characteristics seem to be unfavourable for analysing a common type of enrichment trial where a continuous biomarker is used as selection criterion. Researchers typically use the first stage data to determine a threshold and recruit in the second stage only participants whose biomarker passes this hurdle  \parencite{friede2012conditional, stallard2014adaptive, rosenblum2016group, lai2019adaptive, stallard_adaptive_2023}. However, if we make additional assumptions such as a monotone relationship between the biomarker and treatment effect, some of the ``first-stage randomness'' can be retained and used for conducting inference. We will investigate this scenario in follow-up work.


Third, drop-out units, which are commonly observed in clinical trials, pose challenges for drawing valid inference. The particular difficulty of conducting randomization tests lies in the inability to impute the missing outcomes of drop-out units. Solutions to this problem include model-based or non-informative outcome imputation and reweighting the treatment assignments probabilities among the
subjects with observed outcomes based on the outcome missingness probabilities \parencite{edgington2007randomization, rosenberger_randomization_2019, ivanova2022randomization, heussen2023randomization}.
% and shifting to sensitivity analysis to provide upper bounds for the p-values.
If the missingness is independent of the outcomes but possibly influenced by the treatment administered (analogous to the missing at random mechanism), we can extend our proposal to incorporate the missingness following the path of reweighting.
The resulting p-values will be valid for finite samples if the mechanism of missingness is known, or valid asymptotically if the missing mechanism can be consistently estimated.





%\paragraph{Multi-armed Bandit Problems} This class of models provides a formal decision framework for optimally allocating resources to different competing uses under uncertainty. One may imagine a gambler who tries to allocate their money to different slot machines -- or rather one-armed bandits -- with unknown win probabilities over several rounds of playing. Work on this problem stretches back to \textcite{thompson_likelihood_1933} and the seminal proposal of the Gittins index by \textcite{gittins_dynamic_1974,gittins_dynamic_1979}.These and other proposed algorithms trade off exploring the success probabilities against exploiting the most profitable bandit.

%Similarly, in clinical trials the multi-armed bandit framework is helpful to conceptualize the balance between exploring the effectiveness of all tested treatments and assigning many patients to the most beneficial one as well as other secondary objectives. For more details on tailoring bandit algorithms to clinical settings we refer to \textcite{villar_multi-armed_2015,villar_responseadaptive_2015} and \textcite{villar_covariate-adjusted_2018}.

%Analysing data from such adaptive strategies is challenging due to the complex induced dependence structure between different treatment assignments. Therefore, most proposed approaches invoke general assumptions on the bandit algorithm rather than using \zg{use?} knowledge of the specific allocation strategy that was deployed, for instance \textcite{zhang_inference_2020}, \textcite{hadad_confidence_2021} and \textcite{howard_time-uniform_2021}.

% \include{continuous-covariate}

\paragraph{Continuous selection statistic} 
In enrichment trials, continuous random variables like biomarkers are employed during the interim analysis after the first stage to identify the subpopulation to focus on in the second stage. Conceptually, there is no obstacle to apply our method to this type of selection rules, however, our proposal might not be more powerful compared to simply applying the randomization test to the second-stage units.
In the extreme case, if each first-stage treatment assignment leads to a different value of the selection statistic, then our proposal essentially reduces to the second-stage randomization test.
In addition, the proportion of treatment assignments yielding the exact value of a continuous selection statistic is typically small, bringing in challenges in computation, especially when rejection sampling is used.

Fortunately, if there is a prior belief that a larger treatment effect will be associated with a more positive biomarker, and the decision after the first stage is to enrich to include patients whose biomarker passes a data-driven threshold \cite{friede2012conditional, stallard2014adaptive, rosenblum2016group, lai2019adaptive, stallard_adaptive_2023}, then there is a delicate conditional randomization test which not only achieves the maximum possible power gain but also remains computationally feasible. 
We will investigate this scenario in a follow-up work.



\paragraph{Drop-out units}
Drop-out units, commonly observed in clinical trials, introduce challenges for drawing valid inference. Particularly, the difficulty of conducting randomization tests with drop-out units lies in the inability to impute values of the units with missing outcomes. Solutions to this problem include model-based or non-infomative outcome imputation and reweighting the treatment assignments probabilities among the
subjects with observed outcomes based on the outcome missingness probabilities \cite{edgington2007randomization, rosenberger_randomization_2019, ivanova2022randomization, heussen2023randomization}.
% and shifting to sensitivity analysis to provide upper bounds for the p-values. 


If the missingness is independent of the outcomes but possibly influenced by the treatment administered (analogous to the missing at random mechanism), we can extend our proposal to incorporate the missingness following the path of reweighting.
The resulting p-values will be valid for finite samples if the mechanism of missingness is known, or valid asymptotically if the missing mechanism can be consistently estimated.


\printbibliography

\appendix

\include{appendix}


\section{Details of the Simulation Study on Hold-out Units}
We use the data-generating mechanism of the two-stage enrichment trial as described in Section~\ref{sec:simulation-study} and modify it as follows.

First, we consider the common scenario that there is treatment effect heterogeneity between groups. To this end, we generate the potential outcomes as $Y_i(1) = Y_i(0)+1$ for participants with low genetic risk and as $Y_i(1) = Y_i(0)$ for participants with high genetic risk; $Y_i(0)$ are i.i.d.\ draws from a standard normal distribution. Hence, the treatment effect in the former group is $1$ and $0$ in the latter.

Second, we lower the number of recruited patients to 16 in the first and second stage each. This allows us to precisely compute the p-values for different treatment effects $\tau$ without the need for a Monte Carlo approximation. Therefore, we can exclude numerical errors as a cause of our findings.

Third, \taf{STOPPED HERE}


Since we aim to compare inference under two different selection rules, we only consider scenarios where both rules choose the same null hypothesis. Otherwise the homogeneous treatment effect would refer to different sets of participants.

Seeds





==> previousMay2024.tex <==
% previous
Let $\lambda(Z_1)$ be the selection rule that maps the stage 1 treatment assignment $Z_1$ to the biomarker threshold.
If $\lambda(w)$ is an injection, then the CRT conditional on $\lambda(Z_1)$ is equivalent to conditional on the full $Z_1$, and the CRT reduces to the RT 2nd :(


We consider a set of selection rules which are likely to produce a good-quality threshold and leave a considerable amount of randomness in stage 1 to empower the CRT.
Without loss of generality, we assume $X_i$ are ordered increasingly. 
For the notation simplicity, we drop the subscript $1$ in $Z_1$ and use $W$ to denote the treatment assignment in stage 1.
Let $\lambda^* := \inf \{X_i: Y_i(1) - Y_i(0) \ge 0\}$ be the oracle biomarker threshold which has access to the entire science table.
Define the filtration
\begin{align*}
    \calF_j: = \sigma\{(Z_i)_{i \le j}, (Y_i)_{i \le j},(X_i)_{i \in [N]}\}.
\end{align*}
We consider the class of thresholding rules $\lambda(w) = X_{T(w)}$, where $T(W)$ is a stopping time adapted to $\calF_j$, i.e., $\{T(W) \le j \} \in \calF_j$.
One example of the stopping time applies the two-sample t-test to the units in a rolling window of the biomarkers,
\begin{align*}
    T(W) 
    &= \inf\left\{j: 
    \frac{{p}_{1,j} - {p}_{0,j}}{\hat{\sigma}_{j}\sqrt{\frac{1}{n_{1,j}} + \frac{1}{n_{0,j}}}} \ge q_{h-2, 1 -\alpha}, n_{1,j} = \sum_{j-h+1}^j Z_i, n_{0,j} = \sum_{j-h+1}^j (1-Z_i), \right. \\
&\left.
\qquad \qquad  
{p}_{1,j} 
= \frac{\sum_{i=j-h+1}^j Z_i Y_i}{n_{1,j}}, {p}_{0,j}
= \frac{\sum_{i=j-h+1}^j (1-Z_i) Y_i}{n_{0,j}}, \right.\\ 
&\left.
\qquad \qquad  
\hat{\sigma}_j = \sqrt{\frac{n_{1,j} {p}_{1,j}(1-{p}_{1,j}) + n_{0,j} {p}_{0,j}(1-{p}_{0,j})}{n_{1,j} + n_{0,j} - 2}}
\right\},
\end{align*}
where $h$ denotes some window-size, and $q_{h-2, 1 -\alpha}$ denotes the $1-\alpha$ quantile of the t-distribution with $h-2$ degrees of freedom.
\zg{Under the monotone assumption, only the units whose $X_i$ falls in the neighborhood of $\lambda^*$ are the most relevant to determine the threshold. As an implication, the units with $X_i \gg \lambda^*$, who benefit the most from the treatment, are perhaps unnecessary to determine $\lambda^*$, and their randomness can be recycled by CRT. 
% The data-driven threshold $\lambda(W)$ is expected to be close to $\lambda^*$.
}


For such a thresholding rule $\lambda(w)$, let $G(W) = \{Z_{1,i}: X_{1,i} \le \lambda(W)\}$, and we select the hypothesis,
\begin{align*}
    H_{\lambda(W)}: Y_i(1) - Y_i(0) \le 0, \quad i: X_{1,i} > \lambda(W).
\end{align*}
Notice that for the imputability of the science table under $H_{\lambda(W)}$, 
% the potential outcomes of the units whose treatment assignments are included in $G(W)$ can \emph{not} be imputed. 
the CRT p-value is required to condition on $G(W)$, that is 
\begin{align*}
    p(W):=\Prob^*(T(Z^*,W) \leq T(Z,W) \mid W, Z, G(Z^*) = G(W)).
\end{align*}
Note that the smaller  $\lambda(W)$ is, the more stage 1 treatments can be randomized in the CRT. The worst case is $\lambda(W) = |\calZ_1|$, where the CRT is equivalent to the RT 2nd.

